Towards Fixed-Point Formats Determination for Faust Programs

Modern programmable digital signal processing relies on floating-point numbers for their ease of use. Fixed-point number formats have the potential to save resources and improve execution time, but realising this potential burdens the programmer with the need to define each format, at every step of the computation. This article reviews existing methods to automatically determine fixed-point formats, then describes and evaluates the prototype implementation of automatic fixed-point format determination in the Faust compiler.

==> sources/fig/compilation-chain.tex <==
\scalebox{0.6}{
  \begin{tikzpicture}[x=\tkzscalex,y=\tkzscaley]
  
  \node[draw=greentext, text = greentext, circle, fill=greenbg, minimum height = 2*\tkzscaley,text width=2*\tkzscalex,align=center,] (FAUST) at (0,0) {Faust Code};
  
  \node[draw=yellowtext, text=yellowtext, rounded corners=2pt, fill=yellowbg2, text width=2*\tkzscalex, align=center, minimum height = 2*\tkzscaley, right = 0.5*\tkzscalex of FAUST] (SEMANTIC)  {Semantic Phase};
  
  
  \node[text=greentext, draw= greentext, fill=greenbg, ellipse, text width=2.5*\tkzscalex, align=center, minimum height = 2*\tkzscaley, right = 0.5*\tkzscalex of SEMANTIC, inner sep = 2pt] (SIGNAL)  {List of signals in Normal Form};
  
  \node[draw=yellowtext, text=yellowtext, rounded corners=2pt, fill=yellowbg2, text width=2*\tkzscalex, align=center, minimum height = 2*\tkzscaley, right = 0.5*\tkzscalex of SIGNAL] (GENERATION) {Code Generation Phase};
  
  \node[text=redtext, draw= redtext, fill=redbg, ellipse, text width=2.5*\tkzscalex, align=center, minimum height = 2*\tkzscaley, right = 0.5*\tkzscalex of GENERATION, inner sep = 2pt] (IMPLEMENTATION)  {Implemen-tation: C++, js, LLVM\ldots};
  
  
  \draw[->] (FAUST) -- (SEMANTIC);
  \draw[->] (SEMANTIC) -- (SIGNAL);
  \draw[->] (SIGNAL) -- (GENERATION);
  \draw[->] (GENERATION) -- (IMPLEMENTATION);
  
  % \draw[rounded corners = 2pt, fill=yellowbg] (1.5, -1.1) rectangle (10.5, 1.1);
  \scoped[on background layer]{\node [fit=(SEMANTIC)(SIGNAL)(GENERATION), rounded corners = 2pt, fill=yellowbg, draw=yellowtext, inner sep = 5pt] {};}
  
\end{tikzpicture}
}

==> sources/fig/semantic-phase.tex <==
\scalebox{0.6}{
  \begin{tikzpicture}[x=\tkzscalex,y=\tkzscaley]
  
  \node[draw=greentext, text = greentext, circle, fill=greenbg, minimum height = 2*\tkzscaley,text width=2*\tkzscalex,align=center] (FAUST) at (0,0) {Faust Code};
  
  \node[draw=yellowtext, text=yellowtext, rounded corners=2pt, fill=yellowbg2, text width=2*\tkzscalex, align=center, minimum height = 2*\tkzscaley, right = 0.5*\tkzscalex of FAUST] (CALCULUS)  {Evaluation ($\lambda$-calculus)};
  
  
  \node[text=greentext, draw= greentext, fill=greenbg, ellipse, text width=2.5*\tkzscalex, align=center, minimum height = 2*\tkzscaley, right = 0.5*\tkzscalex of CALCULUS, inner sep = 2pt] (CIRCUIT)  {Circuit};
  
  \node[draw=yellowtext, text=yellowtext, rounded corners=2pt, fill=yellowbg2, text width=2*\tkzscalex, align=center, minimum height = 2*\tkzscaley, right = 0.5*\tkzscalex of CIRCUIT] (PROPAGATION) {Symbolic Propagation};
  
  \node[text=greentext, draw= greentext, fill=greenbg, ellipse, text width=2.5*\tkzscalex, align=center, minimum height = 2*\tkzscaley, right = 0.5*\tkzscalex of PROPAGATION, inner sep = 2pt] (SIGNAL)  {List of Signals};
  
  \node[draw=yellowtext, text=yellowtext, rounded corners=2pt, fill=yellowbg2, text width=2*\tkzscalex, align=center, minimum height = 2*\tkzscaley, right = 0.5*\tkzscalex of SIGNAL] (NORM) {Simplifica-tion and Normalisation};
  
  \node[text=greentext, draw= greentext, fill=greenbg, ellipse, text width=2.5*\tkzscalex, align=center, minimum height = 2*\tkzscaley, right = 0.5*\tkzscalex of NORM, inner sep = 2pt] (SIGNAL2)  {List of signals in Normal Form};
  
  
  \draw[->] (FAUST) -- (CALCULUS);
  \draw[->] (CALCULUS) -- (CIRCUIT);
  \draw[->] (CIRCUIT) -- (PROPAGATION);
  \draw[->] (PROPAGATION) -- (SIGNAL);
  \draw[->] (SIGNAL) -- (NORM);
  \draw[->] (NORM) -- (SIGNAL2);
  
  % \draw[rounded corners = 2pt, fill=yellowbg] (1.5, -1.1) rectangle (10.5, 1.1);
  \scoped[on background layer]{\node [fit=(CALCULUS)(CIRCUIT)(PROPAGATION)(SIGNAL)(NORM), rounded corners = 2pt, fill=yellowbg, draw=yellowtext, inner sep = 5pt] {};}
    
\end{tikzpicture}
}

==> sources/tikz-macros.tex <==
\tikzset{
  >=Stealth, % can't stand the default arrows
  multrectangle/.style={draw, fill=black!5},
  generator/.style={draw,align=center,fill=blue!5,rounded corners, minimum width=15ex, minimum height=8ex},
%  hwblock/.style={draw, rectangle, rounded corners=.3, very thick, fill=black!5, font=\sf, minimum height=5ex,align=center},
  hwblock/.style={draw, rectangle, rounded corners=.3, thick, fill=black!2, drop shadow={shadow xshift=.5ex,shadow yshift=-.5ex}, font=\sf, minimum height=5ex,align=center},
  hwregblock/.style={hwblock, fill=blue!10},
  every circuit symbol/.style={hwblock},
  filteradd/.style={hwblock, circle, minimum height=1ex},
  filtermult/.style={hwblock, minimum height=7ex, regular polygon, regular polygon sides=3, shape border rotate=180, inner sep= .2ex},
  hwbus/.style={very thick,>={Stealth[length=6pt]}},
  hwbuslarge/.style={line width=2pt,>={Stealth[length=7pt]}},
  hwbuswhitebackground/.style={line width=4pt,color=white},
  hwwire/.style={thin, >={Stealth[length=4pt]}  },
  hwword/.style={draw, rectangle, minimum height=3ex},
  bitwidth/.style={font=\scriptsize,blue},
  abitwidth/.style={bitwidth,above},
  bbitwidth/.style={bitwidth,below},
  lbitwidth/.style={bitwidth,left},
  rbitwidth/.style={bitwidth,right},
  flopocoClass/.style={font=\small\tt,draw,align=center,rectangle,fill=blue!5,minimum height=3ex},
  flopocoInfo/.style={font=\small,align=center,rectangle, fill=yellow!50,fill opacity=0.5, text opacity=1,rounded corners=10}
}
% Other colors that could be used consistent
\definecolor{normalbitcolor}{rgb}{0,0,0.5}
\definecolor{normalbitfillcolor}{rgb}{0.8,1,0.8}
\definecolor{signbitcolor}{rgb}{0.5,0,0}
\definecolor{signbitfillcolor}{rgb}{1,0.8,0.8}




\newboolean{showbitwidths} 
\setboolean{showbitwidths}{true}
\newcommand{\bitwidth}[3]{ % coordinate, text, [a|b|l|r]
  \ifthenelse{\boolean{showbitwidths}}{
    \draw[bitwidth,ultra thin] (#1) ++(0.5ex, 0.5ex)  -- ++(-1ex, -1ex) ++(0.5ex, 0.5ex)  node[#3bitwidth] {#2};
  }{}
} %

% Shifts in shift-and-add figure
\newcommand{\leftbitshift}[2]{ % coordinate, value
    \draw[font=\small, thick, Latex-] (#1) ++(-2ex, 0)  -- ++(3ex,0)  node[right] {#2};
} %

\newcommand{\rightbitshift}[2]{ % coordinate, value
    \draw[font=\small, thick, Latex-] (#1) ++(2ex, 0)  -- ++(-3ex,0)  node[left] {#2};
} %


\newcommand{\vhdlfile}[2]{ % x,y
  \draw[fill=black!5] (#1,#2) ++(3.5ex, -5ex) -- ++(-7ex,0) -- ++(0,10ex) -- ++(6ex,0)
  -- ++(1ex,-1ex)-- ++(-1ex,0) -- ++(0,1ex) -- ++(1ex,-1ex) -- cycle;%  (vhdl) at (15ex,0ex) {.vhdl};
  \draw (#1,#2) ++(+3.5ex, -5ex) node[above left] {.vhdl};
  \draw (#1,#2) ++(-3.5ex, 0) node(vhdlnode) {};
  \coordinate (vhdl) at (vhdlnode.center);
}


\newcommand{\drawclockinput}[1] { % name of a hwregblock
  \draw(#1.south) ++(0,1) -- (#1.south west); 
  \draw(#1.south) ++(0,1) -- (#1.south east); 
} 
\newcommand{\multtrunc}[3]{ % name, exponent, scale
  \coordinate (#1) at #2;
  \begin{scope}
  \tikzset{x=#3,y=#3}; % scale
  \filldraw[hwblock] (#1) ++(+3,0) -- ++(0,-1) -- ++(-2,-2) -- ++(-4,0)-- ++(0,6)-- ++(6,0) -- cycle;
  \node at (#1) {\large$\times$};
  \coordinate[shift={(0,  -3)}] (#1South) at (#1);  
  \coordinate[shift={(0,  +3)}] (#1North) at (#1);  
  \coordinate[shift={(-3,0)}] (#1West) at (#1);  
  \coordinate[shift={(+3, +1)}] (#1East) at (#1);
  \end{scope}
}
\newcommand{\squaretrunc}[3]{ % name, exponent, scale
  \coordinate (#1) at #2;
  \begin{scope}
  \tikzset{x=#3,y=#3}; % scale
  \filldraw[hwblock] (#1) ++(+3,0) -- ++(0,-1) -- ++(-2,-2) -- ++(-4,0)-- ++(0,6)-- ++(6,0) -- cycle;
  \node at (#1) {\large$x^2$};
  \coordinate[shift={(0,  -3)}] (#1South) at (#1);  
  \coordinate[shift={(0,  +3)}] (#1North) at (#1);  
  \coordinate[shift={(-3,0)}] (#1West) at (#1);  
  \coordinate[shift={(+3, +1)}] (#1East) at (#1);
  \end{scope}
}

\newcommand{\multadd}[3]{ %name, exponent, scale 
  \coordinate (#1) at #2;
  \begin{scope}
  \tikzset{x=#3,y=#3}; % scale
  \filldraw[hwblock] (#1) ++(+3,0) -- ++(0,-1) -- ++(-2,-2) -- ++(-4,0)-- ++(0,6)-- ++(6,0) -- cycle;
  \filldraw[hwblock] (#1) ++(+3,0) -- ++(0,-1) -- ++(+2ex,0) -- ++(0,+4)-- ++(-2ex,0) -- cycle;
  \node at (#1) {\large$\times$};
  \draw (#1) ++(3,1) ++(1ex,0) node{$+$};
  \coordinate[shift={(+3,  +1)}] (#1MultOut) at (#1);  
  \coordinate[shift={(+2ex,  0)}] (#1Out) at (#1MultOut);  
  \coordinate[shift={(-3, +1)}] (#1InMA) at (#1);  
  \coordinate[shift={(-3, -1)}] (#1InMB) at (#1);  
  \coordinate[shift={(0,+2)}] (#1InAddTempSorry) at (#1MultOut);  
  \coordinate[shift={(+1ex,0)}] (#1InAdd) at (#1InAddTempSorry);  
  \end{scope}
}

\newcommand{\mybracket}[3]{% center position, width in bits, height
  \draw[hwword](#1) --  ++($(0.5*#2-.2,0)$)  -- ++(.2,#3);
  \draw[hwword](#1) --  ++($(-0.5*#2+.3,0)$)  -- ++(-.2,#3);
}


%%%%%%%%%%%%%%%%%%%%%%%%%% Macros for drawing fixed-point formats %%%%%%%%%%%%%%%%%%%%%%%%% 

% Select one of the following bit style: rectangle, or circle as in bit heaps
\newcommand{\drawbit}{rectangle +(-1,1)}   % Square bits
%\newcommand{\drawbit}{+(-0.5,0.5) circle[radius=0.4]} % circle bits


\newcommand{\fixpointdot}[1] % posY
{
	\draw[black,fill] (0,#1-0.3) circle [radius=0.1];
}

% This command is to be invoked within a tikzpicture.
% Can be scaled by [x=2ex, y=2ex] etc
\newcommand{\fixpointnumbernodot}[4] % sign, MSB, LSB, posY
{ 
	\foreach \i in {#3,...,#2} {
		\draw (-\i,#4-0.3) \drawbit[normalbitcolor,fill=normalbitfillcolor];
	}
	\ifthenelse{#1=1}{
		\draw (-#2,#4-0.3) \drawbit[signbitcolor,fill=signbitfillcolor];
	} 
	{
		\draw (-#2,#4-0.3) \drawbit[normalbitcolor,fill=normalbitfillcolor];
	}
}

% version without the separation into bits
\newcommand{\fixpointbox}[4] % sign, MSB, LSB, posY
{ 
   \draw[normalbitcolor,fill=normalbitfillcolor] (-#3,#4-0.3) rectangle +(#3-#2-1,1);
 }

 % used in fpacc figures
\newcommand{\fixpointboxtrunc}[5] % sign, MSB, LSB, posY, wlsbcut
{ 
   \draw[normalbitcolor,fill=normalbitfillcolor] (-#5,#4-0.3) rectangle +(#5-#2-1,1);
   \draw[normalbitcolor,fill=normalbitfillcolor,opacity=0.5,fill opacity=0.5] (-#3,#4-0.3) rectangle +(#3-#5,1);
}
  \newcommand{\fixpointnumber}[4] % sign, MSB, LSB, posY
{ 
	\fixpointnumbernodot{#1}{#2}{#3}{#4}
	\fixpointdot{#4};
}

% FIXME doesn't work
\newcommand{\fixpointreal}[4] % sign, MSB, LSB, posY
{ 
	\fixpointnumber{#1}{#2}{#3}{#4}
	\foreach \i in {0,...,9} 
	{ 
		\tikzmath{ \shade=\i*10;} 
		 \draw  (-#3+10-\i,#4-0.3)\drawbit[normalbitfillcolor!\shade,fill=normalbitfillcolor!\shade] ;
	}
		
	% \foreach \i in {1,...,5} {
	%  	\draw (-#3+\i,#4-0.3) \drawbit[shadedbit];
	% }
}

% This command shows the bit positions axis properly for a \fixpointnumber with the same parameters
% Then Florent decided this axis doesn't make sense WRT the real axis and it is better to remove is
\newcommand{\fixpointpositionsaxis}[4] % sign, wMSB, wLSB, posY
{	
	% \draw[->,thick,>=stealth] (-#3+1,#4-1) -- (-#2-3,#4-1);
	% \foreach \i in {#3,...,#2} {
	% 	\draw (-\i-0.5,#4-.8) -- ++(0,-0.4) ;
	% }
  }
  
\newcommand{\fixpointpositions}[4] % sign, wMSB, wLSB, posY
{
  \fixpointpositionsaxis{#1}{#2}{#3}{#4}
	\ifthenelse{#1=1}{
%		\draw (-#2,#4) +(-0.5,0.2) node{\footnotesize $s$};
	}{}
	\foreach \i in {#3,...,#2} {
		\draw[blue] (-\i-0.5,#4-1) node{\footnotesize \i};
	}
  \draw[blue] (-#3-0.5,#4-1) node[right=0.3]{\footnotesize $=\ell$};    
  \draw[blue] (-#2-0.75,#4-1) node[left]{\footnotesize $m=$};
  \draw[blue] (-#2-3, #4-1)  node[left] {\small bit exponent};
}

\newcommand{\integerbitpositions}[4] % sign, wMSB, wLSB, posY
{
  \fixpointpositionsaxis{#1}{#2}{#3}{#4}
	\ifthenelse{#1=1}{
		\draw (-#2,#4) +(-0.5,0.2) node{\footnotesize $s$};
	}{}
	\foreach \i in {#3,...,#2} {
		\draw[blue] (-\i-0.5,#4-1) node{\footnotesize \i};
	}
  \draw[blue] (-#2-3, #4-1)  node[left] {\small bit exponent};
  %\draw[blue] (-#2-1,#4-1) node[left]{\footnotesize $w-1=$};
}
  

% This command shows the bit weights properly for a \fixpointnumber with the same parameters
% Shows the numerical bit weights
  \newcommand{\fixpointweights}[4] % sign, wMSB, wLSB, posY
{	
	\ifthenelse{#1=0}{
		\draw (-#2-0.5,#4+1.5) node {\small $2^{#2}$};
	}{ 
%		\draw[->,thick,>=stealth] (-#2-1.7, #4+1.5) node (w) {\small $-2^{m}$~} ;%-- ++(-1,+1) node[above=-0.5ex] ;
    \draw (-#2-1, #4+1.5) node (w) {\small $-2^{#2}$~} ;
    % TODO resurrect the next line
 %		\draw (-#2+1, #4+1.5) node (w) {\small $~~2^{#2-1}$};
%    \draw[->,thick,>=stealth] (w) -- ++(-1,-1);% -- ++(+1,+1) ;
	}
%	\draw (-0.5, #4+1.5) node {\small $2^0$};
\draw (-#3-0.5,#4+1.5) node {\small $2^{#3}$}; 
  \draw (-#2-3, #4+1.5)  node[left] {\small bit weight};

}


\newcommand{\fixpointallweights}[4] % sign, wMSB, wLSB, posY
{
  \pgfmathtruncatemacro{\lsb}{#3} 
  \pgfmathtruncatemacro{\msb}{#2-#1} 
	\ifthenelse{#1=0}{
		\draw (-#2-0.5,#4+1.5) node {\small $2^{#2}$};
	}{ 
    \draw (-#2-1, #4+1.5) node (w) {\small $-2^{#2}$~} ;
	}
  \foreach \x in {\lsb,...,\msb} {
    \draw (-\x-0.5,#4+1.5) node {\small $2^{\x}$};
    }
  \draw (-#2-3, #4+1.5)  node[left] {\small bit weight};
}


% This command shows the bit weights properly for a \fixpointnumber with the same parameters
% shows the bit weigths as (m,l)
\newcommand{\fixpointweightsml}[4] % sign, wMSB, wLSB, posY
{	
	\ifthenelse{#1=0}{
		\draw (-#2-0.5,#4+1.5) node {\small $2^{m}$};
	}{ 
%		\draw[->,thick,>=stealth] (-#2-1.7, #4+1.5) node (w) {\small $-2^{m}$~} ;%-- ++(-1,+1) node[above=-0.5ex] ;
    \draw (-#2-1, #4+1.5) node (w) {\small $-2^{m}$~} ;
		\draw (-#2+1, #4+1.5) node (w) {\small $~~2^{m-1}$};
%    \draw[->,thick,>=stealth] (w) -- ++(-1,-1);% -- ++(+1,+1) ;
	}
	\draw (-0.5, #4+1.5) node {\small $2^0$};
  \ifthenelse{#3=0}{ %then don't draw this, it overlaps with the 2^0
    }{  \draw (-#3-0.5,#4+1.5) node {\small $2^{\ell}$}; }
  \draw (-#2-3, #4+1.5)  node[left] {\small bit weights};
}


% the two following macros are for the fpacc drawings

% Plots the bits of a given number in a given fixed-point format
\newcommand{\fpsignificand}[4] % wF, integer exponent, posY, integer significand value
{
  \pgfmathsetmacro{\xinit}{#4} 
  \pgfmathsetmacro{\lsb}{#2} 
   \pgfmathtruncatemacro{\msb}{#2+#1} 
   \draw[normalbitcolor,fill=normalbitfillcolor] (-\lsb,#3-0.3) rectangle +(-#1-1,1);
	 \foreach \i [remember=\x as \xlast (initially \xinit)] in {\lsb,...,\msb} {
     \pgfmathtruncatemacro{\t}{\xlast / 2}
     \pgfmathtruncatemacro{\currentbit}{\xlast - 2*\t}
     \pgfmathsetmacro{\x}{\t}
     \draw (-\i-0.5,#3+0.2) node{\footnotesize \currentbit};
   }
}
% Plots the bits of a given number in a given fixed-point format
\newcommand{\fpaccbits}[4] % wF, integer exponent, posY, integer significand value
{
  \pgfmathsetmacro{\xinit}{#4} 
  \pgfmathsetmacro{\lsb}{#2} 
   \pgfmathtruncatemacro{\msb}{#2+#1} 
   \draw[draw=none,normalbitcolor,fill=normalbitfillcolor] (-\lsb,#3-0.3) rectangle +(-#1-1,1);
	 \foreach \i [remember=\x as \xlast (initially \xinit)] in {\lsb,...,\msb} {
     \pgfmathtruncatemacro{\t}{\xlast / 2}
     \pgfmathtruncatemacro{\currentbit}{\xlast - 2*\t}
     \pgfmathsetmacro{\x}{\t}
     \draw (-\i-0.5,#3+0.2) node{\footnotesize \currentbit};
   }
}

%Plots the bits of a given number in a given fixed-point format
\newcommand{\fixpointvalue}[4] % MSB, LSB, posY, value
{
  \pgfmathsetmacro{\xinit}{#4} 
  \pgfmathsetmacro{\lsb}{#2} 
   \pgfmathtruncatemacro{\msb}{#1} 
	 \foreach \i [remember=\x as \xlast (initially \xinit)] in {\lsb,...,\msb} {
     \pgfmathtruncatemacro{\t}{\xlast / 2}
     \pgfmathtruncatemacro{\currentbit}{\xlast - 2*\t}
     \pgfmathsetmacro{\x}{\t}
     \draw (-\i-0.5,#3+0.2) node{\footnotesize \bf \currentbit};
   }
%  \draw(0,0) node {\x}; 
}

% Plots a random string of ones and zeroes - UNTESTED
\newcommand{\fixpointrandomreal}[3] % wMSB, wLSB, posY
{	
	\fixpointdot{#3}
	\foreach \i in {#2,...,#1} {
		\ifthenelse{\i=#1}		{
			\draw (-\i-0.5,#3+0.2) node{\tt \footnotesize 1};
		}		{
			\draw (-\i-0.5,#3+0.2) node{\tt \footnotesize \pgfmathparse{isodd(random(2))}\pgfmathresult};
		}
	}
	
}


\newcommand{\FloatPlotZero} % minExp, maxExp, wF
{
	\draw[red] (0,.15) -- ++(0,-.4) node[below] {\textcolor{red}{0}};	
}


% This is a drawing of the bits centered on the 
\newcommand{\floatformatnotext}[4]{ % h, wE, wF, text
    \pgfmathsetmacro{\posy}{-3.5*#1} 
    \pgfmathsetmacro{\mywE}{2*#2}  
    \pgfmathsetmacro{\mywF}{2*#3} 
    \foreach \x in {-#2,...,#3} {
      \draw[black!30](2*\x,\posy) -- ++(0,2);
    }
    \draw[fill=magenta, fill opacity=0.3](0,\posy) rectangle ++(-\mywE,2);
    \draw[fill=signbitfillcolor, fill opacity=0.3](-\mywE,\posy) rectangle ++(-2,2);
    \draw[fill=normalbitfillcolor, fill opacity=0.3](0,\posy) rectangle ++(\mywF,2);
    \draw (-\mywE,\posy) ++ (-3,1) node[left]{\small \bf #4};
  }
\newcommand{\floatformat}[4]{ % h, wE, wF, text
    \pgfmathsetmacro{\posy}{-3.5*#1} 
    \pgfmathsetmacro{\mywE}{2*#2}  
    \pgfmathsetmacro{\mywF}{2*#3} 
    \foreach \x in {-#2,...,#3} {
      \draw[black!30](2*\x,\posy) -- ++(0,2);
    }
    \draw[fill=magenta, fill opacity=0.3](0,\posy) rectangle ++(-\mywE,2) node[opacity=1,midway]{\small $E$};
    \draw[fill=signbitfillcolor, fill opacity=0.3](-\mywE,\posy) rectangle ++(-2,2) node[opacity=1,midway]{\small $s$};;
    \draw[fill=normalbitfillcolor, fill opacity=0.3](0,\posy) rectangle ++(\mywF,2) node[opacity=1,midway]{\small $F$};;
    \draw (-\mywE,\posy) ++ (-3,1) node[left]{\small \bf #4};
  }



\newcommand{\FloatPlotNormals}[4] % wE, wF, minExp, maxExp
{
  \pgfmathsetmacro{\wE}{#1} ; 
  \pgfmathsetmacro{\wF}{#2} ; 
  \pgfmathtruncatemacro{\minexp}{#3};  %
  \pgfmathtruncatemacro{\maxexp}{#4}; 
	\pgfmathsetmacro{\pwE}{exp(ln(2)*\wE)+.5}; % rounding by +.5 and truncation
	\pgfmathtruncatemacro{\pwF}{exp(ln(2)*\wF)+.5}; % rounding by +.5 and truncation

  % debug info, beause tex's fix point math is very inaccurate
%  \draw[red](-4,.5) node{$e_{\min}$:\minexp} ++ (2,0) node{$e_{\max}$:\maxexp} ++ (2,0) node{$2^\wF$:\pwF}++ (1,0) node{};

  \foreach \e in {\minexp,...,\maxexp} {
    \pgfmathtruncatemacro{\xscaled}{\pwE*(exp(ln(2)*\e))+0.5}; % force a rounding here for accuracy
    \pgfmathsetmacro{\x}{\xscaled/\pwE}; 
    \draw[thin] (\x,-.15) -- ++(0, .5);%; ++(0,0.5*\e) node[blue, above] {\x} ++(0,.5) node[above, red]{\e};
    \draw[thin] (-\x,-.15) -- ++(0, .5);%; ++(0,0.5*\e) node[blue, above] {\x} ++(0,.5) node[above, red]{\e};
    
    \pgfmathtruncatemacro{\pwFm}{\pwF-1}; 
    \foreach \f in {1,...,\pwFm} {
    \pgfmathsetmacro{\xu}{\x+\f*\x/\pwF}; 
    \draw[thin] (\xu,-.15) -- ++(0, .3);
    \draw[thin] (-\xu,-.15) -- ++(0, .3);% node[blue, above]{\xu}++(0, .3) node[red, above]{\f};
    }
  }
}

\newcommand{\FloatPlotIEEENormals}[2] % wE, wF
{
  \pgfmathsetmacro{\wE}{#1} ; 
  \pgfmathsetmacro{\wF}{#2} ; 
  \pgfmathtruncatemacro{\pwE}{exp(ln(2)*\wE)+.5}; % rounding by +.5 and truncation
  \pgfmathtruncatemacro{\minexp}{2-\pwE/2};  %
  \pgfmathtruncatemacro{\maxexp}{\pwE/2-1};
  \FloatPlotNormals{\wE}{\wF}{\minexp}{\maxexp}
}

\newcommand{\FloatPlotIEEESubnormals}[2] % wE, wF
{
  \pgfmathsetmacro{\wE}{#1} ; 
  \pgfmathsetmacro{\wF}{#2} ; 
  \pgfmathtruncatemacro{\pwE}{exp(ln(2)*\wE)+.5}; % rounding by +.5 and truncation
  \pgfmathtruncatemacro{\minexp}{2-\pwE/2};  %
  \pgfmathtruncatemacro{\pwFm}{\pwF-1}; % rounding by +.5 and truncation
  \pgfmathtruncatemacro{\xscaled}{2*\pwE*(exp(ln(2)*\minexp))+0.5}; % force a rounding here for accuracy
  \pgfmathsetmacro{\x}{\xscaled/(2*\pwE)}; 

  \foreach \f in {0,...,\pwFm} {
    \pgfmathsetmacro{\xu}{\f*\x/\pwF}; 
    \draw[thick,red] (\xu,-.15) -- ++(0, .3);
    \draw[thick,red] (-\xu,-.15) -- ++(0, .3);% node[blue, above]{\xu}++(0, .3) node[red, above]{\f};
    }
}

\newcommand{\FloatPlotFlopoco}[2] % wE, wF, maxrange to be displayed
{
  \pgfmathsetmacro{\wE}{#1} ; 
  \pgfmathsetmacro{\wF}{#2} ; 
  \pgfmathtruncatemacro{\pwE}{exp(ln(2)*\wE)+.5}; % rounding by +.5 and truncation
  \pgfmathtruncatemacro{\pwF}{exp(ln(2)*\wF)+.5}; % rounding by +.5 and truncation
  \pgfmathtruncatemacro{\minexp}{-\pwE/2+1};  %
  \pgfmathtruncatemacro{\maxexp}{\pwE/2};
  % debug info, beause tex's fix point math is very inaccurate
  % \draw[red](-4,1) node{\minexp} ++ (2,0) node{\maxexp} ++ (2,0) node{\pwE}++ (1,0) node{\pwF};
  \FloatPlotNormals{\wE}{\wF}{\minexp}{\maxexp}
  \draw[red,thin] (0,-.3) -- (0, .4);
}


